Dataset Distillation via Adversarial Prediction Matching

Dataset distillation is the technique of synthesizing smaller condensed datasets from large original datasets while retaining necessary information to persist the effect. In this paper, we approach the dataset distillation problem from a novel perspective: we regard minimizing the prediction discrepancy on the real data distribution between models, which are respectively trained on the large original dataset and on the small distilled dataset, as a conduit for condensing information from the raw data into the distilled version. An adversarial framework is proposed to solve the problem efficiently. In contrast to existing distillation methods involving nested optimization or long-range gradient unrolling, our approach hinges on single-level optimization. This ensures the memory efficiency of our method and provides a flexible tradeoff between time and memory budgets, allowing us to distil ImageNet-1K using a minimum of only 6.5GB of GPU memory. Under the optimal tradeoff strategy, it requires only 2.5$\times$ less memory and 5$\times$ less runtime compared to the state-of-the-art. Empirically, our method can produce synthetic datasets just 10% the size of the original, yet achieve, on average, 94% of the test accuracy of models trained on the full original datasets including ImageNet-1K, significantly surpassing state-of-the-art. Additionally, extensive tests reveal that our distilled datasets excel in cross-architecture generalization capabilities.

==> exps_ori.tex <==


\section{Experiments}
%In this section, we first compare our proposed framework with state-of-the-art solutions of dataset distillation along different distilling protocols. To emphasize the practicability, we illustrate that the synthetic data can be generated distributively and then merged by our proposed framework without a significant performance decline. We then exhibit the superior performance of our generated synthetic data in the cross-architecture generalization ability. After that, we conduct comprehensive ablation studies to learn the influence of hyper-parameters. Finally, we apply our generated synthetic dataset to a practical neural architecture search task to demonstrate its reliability.
\subsection{Experimental Setups}
%\subsubsection{Datasets.}
\textbf{Datasets.\quad}We evaluate the performance of our method on distilling four benchmark datasets, including CIFAR-10/100~\citep{cifar}, Tiny ImageNet~\citep{le2015tiny} and ImageNet-1K~\citep{DBLP:journals/ijcv/RussakovskyDSKS15}. Notably, following the protocol of \citet{zhou2022dataset} and \citet{DBLP:conf/icml/CuiWSH23}, we resize the resolution of ImageNet-1K images to $64\times64$ in our evaluations for fair comparison. We provide further detailed information of benchmark datasets in Appendix \ref{app:datasets}.

\textbf{Evaluation Setup and Baselines.\quad}We employ several recent distillation frameworks as baselines including a short-term gradient matching method Data Siamese Augmentation (DSA) \citep{DBLP:conf/icml/ZhaoB21}, a feature distribution matching method Distribution Matching (DM) \citep{DBLP:journals/corr/abs-2110-04181}, two bi-level-optimization-based methods which are FRePo~\citep{zhou2022dataset} and RCIG~\citep{DBLP:conf/icml/LooHLR23}, and three training trajectory matching methods which are Matching Training Trajectory (MTT)~\citep{DBLP:conf/cvpr/Cazenavette00EZ22b} and its two variations TESLA \citep{DBLP:conf/icml/CuiWSH23} and Flat Trajectory Distillation (FTD) \citep{DBLP:conf/cvpr/DuJTZ023}. 

%Further, HaBa \citep{DBLP:journals/corr/abs-2210-16774} recently proposed a new setup for the dataset distillation, which is known as the dataset factorization that the tested synthetic samples are replaced by the outputs of several trained hallucination networks fed with optimized base samples. Haba shows its superior performances by generally boosting existing frameworks. We also investigate the performance of our method combined with Haba and compare it with MTT+Haba which achieves state-of-the-art performance among multiple benchmark tests.
\textbf{Evaluation Metrics.\quad}To evaluate compared methods, we adhere to the standard protocol prevalent in the existing literature. We train 5 randomly initialized networks from scratch over the distilled dataset and evaluate their performances by reporting the mean and standard deviation of their accuracy on the test set. We use the terminology ``IPC'' (an acronym for ``images per class'') in dataset distillation to indicate the size of distilled datasets. Specifically, we examine an IPC of 50/500/1000 for CIFAR-10 and an IPC of 10/50/500 for CIFAR-100, Tiny ImageNet, and ImageNet-1K.

% And for the dataset factorization, we follow the setup suggested by HaBa that set the number of bases per class ($bpc$) as $ipc$ minus 1 in each configuration when $ipc$ is greater than 1, to 
%offset the storage cost of hallucinator networks.
%\subsubsection{Implementation Details.}
\textbf{Implementation Details.\quad}We implement our method based on the procedure of Algorithm \ref{alg:framework}. Specifically, we set the teacher number of $\{\theta^{\mT}\}$ as 100 to be fairly compared with MTT and its variations TESLA and FTD. We set the distance metric $d$ by $L_1$ distance, the running round $R=2,500$, the number of checkpoints $K=5$ and the coefficient of cross-entropy regularizer $\alpha=0.1$ by default. Further details of our hyper-parameter setup and guidelines are in Appendix \ref{app:hyper}.  
%Manhattan distance is employed as the default distance metric. We also investigate performances achieved by several other distance metrics in Appendix \ref{sec:dist}.
% Follow \citep{DBLP:journals/corr/abs-2210-16774}, we also employ 5 hallucination networks for combing with HaBa. 
% More details about our hyperparameter setup can be found in Appendix \ref{}. 
% And detailed information on combing HaBa with our method can be investigated in Appendix \ref{}. 
For a fair comparison, we stay with all the compared precedents to adopt the 3-layer ConvNet architecture \citep{DBLP:conf/cvpr/GidarisK18} for distilling CIFAR-10 and CIFAR-100, and extend to the 4-layer ConvNet for Tiny ImageNet and ImageNet-1K. Moreover, we also employ ZCA whitening for CIFAR-10 and CIFAR-100 as done by previous works \citep{zhou2022dataset,DBLP:conf/icml/LooHLR23,DBLP:conf/cvpr/Cazenavette00EZ22b,DBLP:conf/cvpr/DuJTZ023,DBLP:conf/icml/CuiWSH23}.
All the experimental results of our method can be obtained on one  RTX4090 GPU, including the extensive ImageNet-1K dataset.



\subsection{Comparison to State-of-the-art}\label{sec:comp-sota}
\textbf{Evaluation on ConvNets.\quad}As illustrated by Table~\ref{tab:comp}, our method demonstrates superior performance than all the baselines among all the evaluation scenarios. Notably, ConvNet models trained on our distilled datasets, which are just $10\%$ the size of the original, manage to achieve, on average, $96\%$ of the test accuracies of models trained on the full CIFAR-10, CIFAR-100, and Tiny ImageNet. Conversely, models trained on equivalent-sized random subsets can only reach $58\%$, while the state-of-the-art trajectory matching framework, FTD, achieves a maximum of $87\%$.
Specifically, the average test accuracies of our method surpass those of FTD by $3.1\%$ on CIFAR-10, $2.1\%$ on CIFAR-100, and $5.8\%$ on Tiny ImageNet. Compared to the state-of-the-art bi-level optimization framework RCIG, our framework not only exhibits superior performances at a smaller IPC but also demonstrates feasibility and effectiveness when generating synthetic sets with a larger IPC. Furthermore, thanks to the memory efficiency of our adversarial prediction matching framework, our method stands as one of the only two capable of successfully distilling the extensive ImageNet-1K dataset, and it additionally exceeds the competitor, TESLA, by $4.4\%$ on average.
A visualization study of our synthetic data is shown in Appendix \ref{app:visual}.

\textbf{Cross-Architecture Generalization.\quad}In Table \ref{tab:cross}, we assess the generalization performance of datasets distilled by our method and by several representative baselines, including DSA, DM, RCIG, and FTD, on unseen model architectures over CIFAR and Tiny ImageNet with an IPC of 50.
We utilize three different neural network architectures for evaluation: VGG11~\citep{DBLP:journals/corr/SimonyanZ14a}, ResNet18~\citep{DBLP:conf/cvpr/HeZRS16} and Vision Transformer (ViT)~\citep{DBLP:conf/iclr/DosovitskiyB0WZ21}. Those models are widely employed for cross-architecture evaluations of recent dataset distillation works~\citep{DBLP:conf/nips/CuiWSH22,DBLP:conf/icml/CuiWSH23,DBLP:conf/cvpr/Cazenavette00EZ23}.
 The results demonstrate that models learned with our synthetic data have superior performances than models trained on datasets synthesized by other baselines. Additionally, compared to the results on ConvNet shown in Table \ref{tab:comp}, we surprisingly noticed larger performance improvements of our method to the state-of-the-art FTD method across multiple unseen models. Moreover, our results obtained on ResNet18 even exceed  the results obtained on ConvNet when testing on CIFAR-100 and Tiny ImageNet.The remarkable transferability demonstrates that our method is more capable of capturing the essential features for learning.
We also report the generalization result of our distilled dataset of ImageNet-1K  in Appendix \ref{app:cag1k}.
\begin{table*}[t]  
	\tiny
	\centering  
	\caption{Comparison of the test accuracy (\%) between ours and other distillation methods on CIFAR10/100, Tiny ImageNet and ImageNet-1K datasets. Entries marked as absent are due to scalability issues. See Appendix \ref{app:issuse} for detailed reasons.}    
	\begin{tabularx}{\linewidth}{>{\centering\arraybackslash}p{1.05cm}>{\centering\arraybackslash}p{0.4cm}|ccccccccc|>{\centering\arraybackslash}p{0.7cm}}  \toprule    Dataset & IPC   & Random & DSA   & DM    & FRePo & RCIG  & MTT   & TESLA & FTD   & \textbf{Ours} & Whole \\  \midrule  \multirow{3}[0]{*}{CIFAR-10} & 50    & 50.2±0.5 & 60.6±0.5 & 63.0±0.4 & 71.7±0.2 & 73.5±0.3 & 71.6±0.2 & 72.6±0.7 & 73.8±0.2 & \textbf{75.0±0.2} & \multirow{3}[0]{*}{85.6±0.2} \\          & 500   & 71.9±0.3 & -     & 74.3±0.2 & -     & -     & 78.6±0.2 & 78.4±0.5     & 78.7±0.2 & \textbf{83.4±0.3} &  \\          & 1000  & 78.2±0.3 & -     & 79.2±0.2 & -     & -     & 79.7±0.2 & 80.3±0.3 & 81.2±0.2 & \textbf{84.6±0.2} &  \\   \midrule  \multirow{3}[0]{*}{CIFAR-100} & 10    & 14.4±0.5 & 32.3±0.3 & 29.7±0.3 & 42.5±0.2 & 44.1±0.4 & 40.1±0.4 & 41.7±0.3 & 43.4±0.3 & \textbf{44.6±0.3} & \multirow{3}[0]{*}{56.8±0.2} \\          & 50    & 30.5±0.3 & 42.8±0.4 & 43.6±0.4 & 44.3±0.2 & 46.7±0.3 & 47.7±0.2 & 47.9±0.3 & 50.7±0.3 & \textbf{53.3±0.2} &  \\          & 100   & 43.1±0.2 & 44.7±0.2 & 47.1±0.4 & -     & 47.4±0.3 & 50.3±0.1 & 51.1±0.3     & 52.8±0.3 & \textbf{55.2±0.2} &  \\   \midrule  \multirow{3}[0]{*}{Tiny ImageNet} & 10    & 4.8±0.3 & 15.9±0.2 & 12.9±0.4  & 25.4±0.2 & 29.4±0.2 & 23.2±0.2 & 14.1±0.3     & 24.5±0.2 & \textbf{30.0±0.3} & \multirow{3}[0]{*}{40.0±0.4} \\          & 50    & 15.1±0.3 & 21.6±0.3 & 21.2±0.3 & -     & -     & 28.0±0.3 & 33.4±0.5     & 31.5±0.3 & \textbf{38.2±0.4} &  \\          & 100   & 24.3±0.3 & -     & 29.4±0.2 & -     & -     & 33.7±0.6 & 34.7±0.2     & 34.5±0.4 & \textbf{39.6±0.2} &  \\   \midrule  \multirow{3}[0]{*}{ImageNet-1K} & 10    & 4.1±0.1 & -     & -     & -     & -     & -     & 17.8±1.3 & -     & \textbf{24.8±0.2} & \multirow{3}[0]{*}{37.2±0.5} \\          & 50    & 16.2±0.8 & -     & -     & -     & -     & -     & 27.9±1.2 & -     & \textbf{30.7±0.3} &  \\          & 100   & 19.5±0.5 & -     & -     & -     & -     & -     & 29.2±1.0     & -     & \textbf{32.6±0.3} &  \\    \bottomrule
	\end{tabularx}%  
	\label{tab:comp}%
\end{table*}%

%We attribute the superior performance of our method to the fact that, unlike previous frameworks, our framework does not aim to make the models trained on the synthetic set accurately predict on a subset of the original data or mimic the model behaviors induced by a subset of the original data, such as gradients. Instead, it treats synthetic data as "hard samples" that effectively assist models in aligning predictions with models trained on original data. 


%\begin{figure}[ht]
%	\begin{center}
%		\centerline
%		{\includegraphics[width=0.48\textwidth]{figs/merged_batches.png}}
%		\caption{The merging effectiveness comparison demonstrated by the training performances of merged synthetic datasets varying with the number of distributively generated batches.}
%		\label{fig:merge}
%	\end{center}
	
%\end{figure}


\subsection{Memory and Time Efficiency Analysis}\label{sec:efficiency}
{\textbf{High Efficiency for Distilling ImageNet-1K.}\quad}To empirically evident the superiorities of the memory complexity and the flexible tradeoff between runtime and memory usage we discussed in Section \ref{sec:sup}, we compare our method with TESLA, which exhibits the optimal memory complexity among trajectory matching frameworks, for distilling ImageNet-1K with an IPC of $50$. We conduct tests on a Tesla A100 GPU (80GB) for a fair comparison.  Figure \ref{fig:memory} represents the averaged peak memory usage and runtime per iteration over 50 rounds collected by running algorithms with the reported default hyper-parameters for obtaining the results shown in Table \ref{tab:comp}. Both methods set the mini-batch size for updating synthetic samples in each iteration as $500$. However, our method allows for an equivalent update by distributing the updates of 500 samples across multiple segments. For instance, “Segment-100” implies dividing 500 samples into five parts and updating sequentially. Through this approach, our method can flexibly tradeoff memory usage and runtime, enabling the distillation of ImageNet-1K with merely 6.5GB of memory and achieving superior distillation performance. Additionally, we observe that even when updating 500 samples at once, our method consumes $2.5\times$  less memory than Tesla. Given that the default running iteration of Tesla is double ours, our overall runtime is only one-fifth of theirs.

{\textbf{Parallelizability of Dataset Distillation.}\quad}To further enhance productivity, a logical approach is to divide the generation of a synthetic dataset and allocate it to multiple workers for parallel execution without compromising effectiveness. We refer to this feature as the parallelizability of dataset distillation methods. We evaluate this feature of our method and several representative frameworks including DM, FRePo and MTT in Figure \ref{fig:merge}. Specifically, we separately craft 10 groups of synthetic data with an IPC of 50 for CIFAR-10 and 5 groups with an IPC of 10 for Tiny ImageNet. We can see from the figure that the performances of models attained on our synthetic datasets persistently increase with the growing number of merged groups. Moreover, we are the only framework that can achieve equivalent performances as the original results shown in Table \ref{tab:comp}. This indicates that, unlike other frameworks, running our method in parallel does not capture repetitive or redundant features.

% Table generated by Excel2LaTeX from sheet 'Sheet1'
%  Absent entries of RCIG are attributed to the inability to distil Tiny ImageNet with an IPC of 50.
\begin{table}[t]  
	\tiny
	\centering  
	\caption{Cross-architecture generalization performance in test accuracy (\%) of synthetic datasets distilled for CIFAR-10/100 and Tiny ImageNet at an IPC of 50.}    
	\begin{tabular}{c|c|cccccc}
		%		{c|c|cccccc}     
		\toprule  Dataset   &    Model   & Random & DSA   & DM    & RCIG  & FTD   & \textbf{Ours} \\  \midrule  \multirow{3}[0]{*}{CIFAR-10} & VGG11 & 46.7±0.6 & 51.0±1.1 & 59.2±0.8 & 47.9±0.3 & 59.1±0.2 & \textbf{65.8±1.0} \\          & ResNet18 & 48.1±0.3 & 47.3±1.0 & 57.5±0.9 & 59.5±0.2 & 64.7±0.3 & \textbf{69.2±0.8} \\          & ViT   & 38.9±0.6 & 22.6±1.0 & 27.2±1.6 & 27.7±0.8 & 38.7±0.9 & \textbf{42.2±1.1} \\  \midrule  \multirow{3}[0]{*}{CIFAR-100} & VGG11 & 28.4±0.3 & 29.8±0.1 & 34.6±0.4 & 36.7±0.1 & 42.5±0.2 & \textbf{46.6±0.2} \\          & ResNet18 & 41.0±0.8 & 41.7±0.7 & 37.7±0.5 & 36.5±0.4 & 48.4±0.1 & \textbf{55.2±0.3} \\          & ViT   & 25.5±0.2 & 27.4±0.3 & 28.2±0.6 & 15.7±0.6 & 30.2±0.5 & \textbf{35.2±0.6} \\   \midrule \multirow{3}[0]{*}{Tiny ImageNet} & VGG11 & 21.1±0.3 & 21.5±0.3 & 22.0±0.4 & -     & 27.2±0.3 & \textbf{35.1±0.1} \\          & ResNet18 & 30.7±0.8 & 30.9±1.1 & 20.3±0.4 & -     & 35.7±0.6 & \textbf{40.2±0.2} \\          & ViT   & 17.4±0.6 & 18.6±0.3 & 18.1±0.4 & -     & 21.5±0.1 & \textbf{24.5±0.8} \\   \bottomrule
	\end{tabular}% 
	\label{tab:cross}%
\end{table}%f


\begin{figure}[t]
	\centering
	\begin{minipage}{0.43\textwidth}  % Adjust the width of the minipage as needed
		\centering
		\includegraphics[width=\linewidth]{figs/memory_time_bar.png} % Adjust the image name and width as needed
		\caption{Flexible tradeoff between memory usage and runtime per iteration of our method compared with TESLA's for distilling ImageNet-1K with an IPC of 50.}
		\label{fig:memory}
	\end{minipage}
	\hspace{0.8cm} % To add space between the two figures
	\begin{minipage}{0.47\textwidth}  % Adjust the width of the minipage as needed
		\centering
		\includegraphics[width=\linewidth]{figs/merged_batches.png} % Adjust the image name and width as needed
		\caption{Test accuracy (\%) varying with merging different numbers of distributively generated sub-batches. IPC of each sub-batch is 50 for CIFAR-10 and 10 for Tiny ImageNet.}
		\label{fig:merge}
	\end{minipage}%
\end{figure}

%\subsection{Cross-Architecture Generalization}
%%Above experiments only demonstrate the capability of our method on the same architecture of ConveNet. Nevertheless, 
%The transferability to generalize across diverse unseen architectures is a pivotal characteristic of distilled datasets \citep{DBLP:journals/corr/abs-2110-04181,zhou2022dataset,DBLP:conf/cvpr/DuJTZ023}. 
%We assess the generalization performance of our distilled datasets and contrast it with datasets generated by representative baselines, including DSA, DM, RCIG, and FTD on CIFAR-10/100 and Tiny ImageNet with an IPC of 50.
%The generation of involved synthetic datasets all relies on the 3-layer ConvNet for distilling CIFAR-10/100 and the 4-layer ConvNet for distilling Tiny ImageNet. For evaluation, we utilize three different neural network architectures: VGG11~\citep{DBLP:journals/corr/SimonyanZ14a}, ResNet18~\citep{DBLP:conf/cvpr/HeZRS16} and Vision Transformer (ViT)~\citep{DBLP:conf/iclr/DosovitskiyB0WZ21}. Those models are widely employed for cross-architecture evaluations of recent dataset distillation works~\citep{DBLP:conf/nips/CuiWSH22,DBLP:conf/icml/CuiWSH23,DBLP:conf/cvpr/Cazenavette00EZ23}.  
%The comparison results are reported in Table \ref{tab:cross}. We can see from the result that models learned with our generated synthetic samples have superior performances than models trained on datasets synthesized by other baselines. Additionally, compared to the results on ConvNet (i.e., the proxy model used for the distillation) shown in Table \ref{tab:comp}, we surprisingly noticed larger performance improvements of our method to the state-of-the-art FTD method in evaluations across multiple unseen models. Moreover, our results obtained on ResNet18 even exceed  the results obtained on ConvNet when testing on CIFAR-100 and Tiny ImageNet.The remarkable transferability demonstrates that our method is more capable of capturing the essential features for learning.
%We also report the generalization result of our distilled dataset of ImageNet-1K  in Appendix \ref{app:cag1k}.


\subsection{Ablation Study} \label{sec:ablation}
%In Figure \ref{subfig:expt} \& \ref{subfig:num}, we explore the effectiveness of the two techniques proposed for enhancing the adversarial framework in Sec. \ref{sec:apm} (). We also investigate the stability of model performances varying with the mini-batch size of synthetic data sampled in each iteration (Figure \ref{subfig:size}) and the hyper-parameter tuning process of the epoch number for updating the model weights over the synthetic data (Figure \ref{subfig:epoch}). 
We study the effectiveness or the influence of the following four components of our method. 
\textbf{Number of Pre-trained Teachers:} To enhance the generalization ability, we propose to match prediction with different teachers sampled from a pre-gathered pool $\{\theta^T\}$.  Figure \ref{subfig:expt} reveals a consistent performance increase with the size of $\{\theta^T\}$, emphasizing the importance of dynamically altering the teacher model to circumvent overfitting to a singular model. 
Notably, the result with $10$ teachers is nearly equivalent to that with $100$ teachers, highlighting the potential for computation and storage resource conservation. 
\textbf{Number of Involved Checkpoints:} As illustrated by Figure \ref{subfig:num}, utilizing $K$ checkpoints in Equation (\ref{eq:loss_u}) improves the performance of only using the last checkpoint. Besides, we observe that setting $K$ larger than 5 will not cause significant changes in the performance, allowing equivalent effectiveness with reduced resources.
\textbf{Mini-Batch Size:} In Sec \ref{sec:sup}, we emphasize that the loss function for updating one synthetic sample is computationally independent of others. 
% This property liberated the optimization for a relatively large synthetic dataset when users have strong demand for the performance of the distilled dataset but with limited GPU memories. 
Fig \ref{subfig:size} shows the invariance of performances of synthetic datasets distilled with different mini-batch sizes $B$. Thus, both memory consumption and runtime of each round can be effectively reduced when the mini-batch size is small. 
% \textcolor{blue}{It should be noticed that the tunn of  the hyperparameters of epoch and learning rate for updating the model over the synthetic set had to be redefined to make the model learn adequately.} 
\textbf{Number of Epoch for the Model Update:} We examine the effect of the epoch number $E$ for training student models on the synthetic dataset in Figure \ref{subfig:epoch}. We can see a significant decrease when $E$ is set higher than $300$. This is because a large $E$ will cause most of the $K$ collected checkpoints to be nearly converged. Thus, condensed features derived by using them as proxies lack sufficient knowledge beneficial for the early stages of model training.
Moreover, we comprehensively study the influence of varying the coefficient of cross-entropy regularizer, $\alpha$, over the four benchmark datasets in Appendix \ref{app:alpha}. 


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t] 
	\centering
	\small
	\caption{Comparison of Spearman's ranking correlation of NAS on CIFAR-10.  Results are obtained from models trained on various distilled datasets with an IPC of 50 (i.e., 1\% of the original dataset) over 200 epochs. For reference, the correlation achieved by training models on the full original dataset for 20 epochs stands at 0.52, albeit requiring $10\times$ the search time than ours.}    
	\begin{tabular}{cccccc}
		\toprule    Random & DSA   & DM    & MTT   & FRePo  & \textbf{Ours} \\   \midrule 0.18±0.06 & 0.12±0.07 & 0.13±0.06 & 0.31±0.01 & -0.07±0.07 & \textbf{0.47±0.03} \\    \bottomrule
	\end{tabular}%  
\label{tab:nas}%
\end{table}%

\begin{figure*}[t]
	\centering
	\subfigure[Teacher number]{
		\label{subfig:expt}
		\begin{minipage}[t]{0.24\linewidth}
			\centering
			\includegraphics[width=1.4in]{figs/output_expt.png}
		\end{minipage}%
	}%
	\subfigure[Checkpoint number]{
		\label{subfig:num}
		\begin{minipage}[t]{0.24\linewidth}
			\centering
			\includegraphics[width=1.4in]{figs/output_ck.png}
		\end{minipage}%
	}%
	\subfigure[Mini-batch size]{
		\label{subfig:size}
		\begin{minipage}[t]{0.24\linewidth}
			\centering
			\includegraphics[width=1.4in]{figs/output_mini.png}
		\end{minipage}%
	}%
	\subfigure[Updating epoch of $\theta^{\mS}$]{
		\label{subfig:epoch}
		\begin{minipage}[t]{0.24\linewidth}
			\centering
			\includegraphics[width=1.4in]{figs/output_epoch.png}
		\end{minipage}%
	}%
	\centering
	\caption{Ablation studies of our method conducted on CIFAR-10 with an IPC of 50.}
	\vspace{-0.2cm}
	\label{fig:ablation}
\end{figure*}

\subsection{Application: Neural Architecture Search}

To explore the practicality of our method, we utilize the distilled datasets as a proxy for the intricate Neural Architecture Search (NAS) task. For this, we adopt the same NAS-Bench-201 task \citep{DBLP:conf/iclr/Dong020}, previously employed by a recent dataset distillation benchmark \citep{DBLP:conf/nips/CuiWSH22}.
Specifically, we randomly sample 100 networks from NAS-Bench-201, in which the search space is comprised of 15,625 networks with ground-truth performances collected by training on the entire training dataset of CIFAR-10 for 50 epochs under 5 random seeds, and ranked according to their average accuracy on a held-out validation set of 10k images. We compare our methods with various baselines including Random (a randomly selected subset), DSA, DM, MTT and FRePo by training the 100 different architectural models over synthetic datasets with an IPC of 50 for 200 epochs. The Spearman’s correlation between the rankings derived from the synthetic datasets and the ground-truth ranking is used as the evaluation metric.
Comparison results are reported in Table \ref{tab:nas}. Notably, due to the inherent variability in training, an average ranking correlation of 0.76 is achieved locally even when adhering to the ground-truth protocol. We can clearly see from the table that the ranking correlation attained by our method markedly surpasses other baselines. Especially, although MTT and FRePo's test accuracies in Table \ref{tab:comp} are on par with ours for an IPC of 50 on CIFAR-10, the efficiency of our method for this NAS task is evident. Moreover, the correlation achieved by training models on the entire original training dataset of CIFAR-10 for 20 epochs is 0.52. However, our distilled datasets deliver comparable performance in just one-tenth of the search time. 
%These observations validate the potential of our method in enhancing the efficiency of NAS tasks.
